Design of a Single-User RIS-Aided MISO System Based on Statistical Channel Knowledge

Reconfigurable intelligent surface (RIS) is considered a prospective technology for beyond fifth-generation (5G) networks to improve the spectral and energy efficiency at a low cost. Prior works on the RIS mainly rely on perfect channel state information (CSI), which imposes a huge computational complexity. This work considers a single-user RIS-assisted communication system, where the second-order statistical knowledge of the channels is exploited to reduce the training overhead. We present algorithms that do not require estimation of the CSI and reconfiguration of the RIS in every channel coherence interval, which constitutes one of the most critical practical issues in an RIS-aided system.

==> test1_tikz.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,1.00000,0.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor3}{rgb}{0.00000,1.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=12.4in,
height=6.357in,
at={(2.08in,0.858in)},
scale only axis,
xmin=-20,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={$\bf{Transmit\:Power\:in\:dB}$},
ymin=0,
ymax=16,
ylabel style={font=\color{white!15!black}},
ylabel={$\bf{User's\:Rate\:[bpcu]}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.136,0.609)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, dashdotted, line width=4.0pt, mark=diamond, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-20	0.0856328101505123\\
-10	0.663134558869106\\
0	2.65825420862607\\
10	5.78579556515837\\
20	9.04407056491944\\
30	12.3172479267124\\
40	15.7270658836213\\
};
\addlegendentry{$\bf{Genie-Aided\:SDR\:Approach\:(Perfect\:CSI)}$}

\addplot [color=mycolor2, dashdotted, line width=4.0pt, mark=triangle, mark options={solid, rotate=90, mycolor2}]
  table[row sep=crcr]{%
-20	0.0199901263594281\\
-10	0.191010318538022\\
0	1.10613037195198\\
10	3.59055065607716\\
20	6.57154145799079\\
30	9.84980249708097\\
40	13.1662752126901\\
};
\addlegendentry{$\bf{SDR\:Approach\:(Imperfect\:CSI)}$}

\addplot [color=green, dashdotted, line width=4.0pt, mark=o, mark options={solid, green}]
  table[row sep=crcr]{%
-20	0.0076090218856916\\
-10	0.0624779925157209\\
0	0.49560472805375\\
10	2.01925549793462\\
20	4.5502395378743\\
30	7.53421236511627\\
40	10.8811736584046\\
};
\addlegendentry{$\bf{Algorithm\:using\:Jensen's\:Inequality\:[9]}$}

\addplot [color=red, line width=5.0pt, mark=o, mark options={solid, red}]
  table[row sep=crcr]{%
-20	0.0237416698777577\\
-10	0.174609305038857\\
0	0.942964010825341\\
10	3.14910053705563\\
20	5.88740850268363\\
30	9.04305469829078\\
40	12.556205018454\\
};
\addlegendentry{$\bf{Algorithm\:2:\:Element-Wise}$}

\addplot [color=mycolor3, dashed, line width=4.0pt]
  table[row sep=crcr]{%
-20	0.001485323377815\\
-10	0.012894606416807\\
0	0.119161278435432\\
10	0.821270900461883\\
20	2.71908261130914\\
30	5.55532442664717\\
40	8.82659676904828\\
};
\addlegendentry{$\bf{Random\:Phase\:Shift}$}

\addplot [color=black, dashed, line width=4.0pt]
  table[row sep=crcr]{%
-20	0.001485323377815\\
-10	0.012894606416807\\
0	0.074161278435432\\
10	0.571270900461883\\
20	2.21908261130914\\
30	5.05532442664717\\
40	8.32659676904828\\
};
\addlegendentry{$\bf{No\:IRS}$}

\addplot [color=blue, line width=5.0pt, mark=diamond, mark options={solid, blue}]
  table[row sep=crcr]{%
-20	0.0192191789497158\\
-10	0.14237156206731\\
0	0.731237139568615\\
10	2.92233654369326\\
20	5.64565107467853\\
30	8.78384319454364\\
40	12.2980683895856\\
};
\addlegendentry{$\bf{Algorithm\:1:\:Gradient\:Descent}$}

\addplot [color=green, line width=4.0pt, mark=diamond, mark options={solid, green}]
  table[row sep=crcr]{%
-20	0.0264445413197507\\
-10	0.224661799317446\\
0	1.28624338053411\\
10	3.98378366268583\\
20	7.05109097636356\\
30	10.3399885476025\\
40	13.7603688983208\\
};
\addlegendentry{$\bf{Two-Timescale\:Optimisation\:with\:Algorithm\:2}$}

\addplot [color=mycolor1, line width=4.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-20	0.0156550530730704\\
-10	0.146954016332464\\
0	0.994931437356182\\
10	3.40483434274334\\
20	6.60175057488962\\
30	9.77482163513496\\
40	13.0106716362337\\
};
\addlegendentry{$\bf{Two-Timescale\:Optimisation\:[7]}$}

\end{axis}

\begin{axis}[%
width=16in,
height=7.8in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> test3.tex <==
% chktex-file 1
% chktex-file 27

\makeatletter

% The keys that the user can provide are all the keys below.

\pgfkeys{
  /pgf/.cd,
  element fill color/.initial=white,
}


\pgfdeclareshape{IRS}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Saved Anchors for each element top left and bottom right xxxxxxxx
  % 
  % The IRS elements are named with single capital letters in a
  % rowwise fashion. That is, element 1-1 is A, element 1-2 is B, and
  % so on.
  % 
  % The width/height of each IRS element is 0.2 of the full IRS
  % width/height. The spacing between elements is 0.04 of the width/height.
  
  % First row
  \savedanchor\elementAtopleft{%
    \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementAbottomright{%
    \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
  \savedanchor\elementBtopleft{%
    \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementBbottomright{%
    \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  \savedanchor\elementCtopleft{%
    \pgfmathsetlength\pgf@x{0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementCbottomright{%
    \pgfmathsetlength\pgf@x{0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  \savedanchor\elementDtopleft{%
    \pgfmathsetlength\pgf@x{0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementDbottomright{%
    \pgfmathsetlength\pgf@x{0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  % Second Row
  \savedanchor\elementEtopleft{%
    \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.22*\shapeheight}
  }

  \savedanchor\elementEbottomright{%
    \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.02*\shapeheight}
  }
  
  \savedanchor\elementFtopleft{%
    \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.22*\shapeheight}
  }

  \savedanchor\elementFbottomright{%
    \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.02*\shapeheight}
  }

  \savedanchor\elementGtopleft{%
    \pgfmathsetlength\pgf@x{0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.22*\shapeheight}
  }

  \savedanchor\elementGbottomright{%
    \pgfmathsetlength\pgf@x{0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.02*\shapeheight}
  }

  \savedanchor\elementHtopleft{%
    \pgfmathsetlength\pgf@x{0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.22*\shapeheight}
  }

  \savedanchor\elementHbottomright{%
    \pgfmathsetlength\pgf@x{0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.02*\shapeheight}
  }

  % Third Row
  \savedanchor\elementItopleft{%
    \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
  }

  \savedanchor\elementIbottomright{%
    \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
  }
  
  \savedanchor\elementJtopleft{%
    \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
  }

  \savedanchor\elementJbottomright{%
    \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
  }

  \savedanchor\elementKtopleft{%
    \pgfmathsetlength\pgf@x{0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
  }

  \savedanchor\elementKbottomright{%
    \pgfmathsetlength\pgf@x{0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
  }

  \savedanchor\elementLtopleft{%
    \pgfmathsetlength\pgf@x{0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
  }

  \savedanchor\elementLbottomright{%
    \pgfmathsetlength\pgf@x{0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
  }

  % Forth Row
  \savedanchor\elementMtopleft{%
    \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
  }

  \savedanchor\elementMbottomright{%
    \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
  }
  
  \savedanchor\elementNtopleft{%
    \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
  }

  \savedanchor\elementNbottomright{%
    \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
  }

  \savedanchor\elementOtopleft{%
    \pgfmathsetlength\pgf@x{0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
  }

  \savedanchor\elementObottomright{%
    \pgfmathsetlength\pgf@x{0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
  }

  \savedanchor\elementPtopleft{%
    \pgfmathsetlength\pgf@x{0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
  }

  \savedanchor\elementPbottomright{%
    \pgfmathsetlength\pgf@x{0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  
  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  % NONE
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{

    \begin{pgfscope}
      % \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
      % \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfpathrectanglecorners
      {\southwest}
      {\northeast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    \begin{scope} % Scope for all IRS elements to make the rounded corners
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/element fill color}}
      
      % IRS Element 1-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementAtopleft}
        {\elementAbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-2
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementBtopleft}
        {\elementBbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-3
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementCtopleft}
        {\elementCbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-4
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementDtopleft}
        {\elementDbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 2-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementEtopleft}
        {\elementEbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}
      
      % IRS Element 2-2
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementFtopleft}
        {\elementFbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 2-3
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementGtopleft}
        {\elementGbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 2-4
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementHtopleft}
        {\elementHbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 3-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementItopleft}
        {\elementIbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 3-2
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementJtopleft}
        {\elementJbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 3-3
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementKtopleft}
        {\elementKbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 3-4
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementLtopleft}
        {\elementLbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 4-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementMtopleft}
        {\elementMbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 4-2
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementNtopleft}
        {\elementNbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 4-3
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementOtopleft}
        {\elementObottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 4-4
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementPtopleft}
        {\elementPbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}
    \end{scope}
    
    % \begin{pgfscope}
    %   \pgfmoveto{\startpoint}
    %   \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
    %   \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
    %   \pgfpathclose
    %   \pgfusepath{stroke,fill}
    % \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "test_irs.tex"
%%% End:
